SpiralNet++: A Fast and Highly Efficient Mesh Convolution Operator

Intrinsic graph convolution operators with differentiable kernel functions play a crucial role in analyzing 3D shape meshes. In this paper, we present a fast and efficient intrinsic mesh convolution operator that does not rely on the intricate design of kernel function. We explicitly formulate the order of aggregating neighboring vertices, instead of learning weights between nodes, and then a fully connected layer follows to fuse local geometric structure information with vertex features. We provide extensive evidence showing that models based on this convolution operator are easier to train, and can efficiently learn invariant shape features. Specifically, we evaluate our method on three different types of tasks of dense shape correspondence, 3D facial expression classification, and 3D shape reconstruction, and show that it significantly outperforms state-of-the-art approaches while being significantly faster, without relying on shape descriptors. Our source code is available on GitHub.

==> SpiralNet++_ A Fast and Highly Efficient Mesh Convolution Operator/conclusions.tex <==
\section{Conclusions}

We explicitly introduce SpiralNet++ to the domain of 3D shape meshes, where data are generally aligned instead of varied topologies, which allows SpiralNet++ to efficiently fuse neighboring node features with local geometric structure information. We further apply this method to the tasks of dense shape correspondence, 3D facial expression classification and 3D shape reconstruction. Extensive experimental results show that our approach are faster and outperform competitive baselines in all the tasks. 


\section{Acknowledgements}

SG and MB were supported in part by the ERC Consolidator Grant No.724228 (LEMAN), Google
Faculty Research Awards, Amazon AWS Machine Learning Research grant, and the Royal Society Wolfson Research Merit award. SZ was partially supported by the EPSRC Fellowship DEFORM (EP/S010203/1) and a Google Faculty Award.
